FEATHER: A Reconfigurable Accelerator with Data Reordering Support for Low-Cost On-Chip Dataflow Switching

The inference of ML models composed of diverse structures, types, and sizes boils down to the execution of different dataflows (i.e. different tiling, ordering, parallelism, and shapes). Using the optimal dataflow for every layer of workload can reduce latency by up to two orders of magnitude over a suboptimal dataflow. Unfortunately, reconfiguring hardware for different dataflows involves on-chip data layout reordering and datapath reconfigurations, leading to non-trivial overhead that hinders ML accelerators from exploiting different dataflows, resulting in suboptimal performance. To address this challenge, we propose FEATHER, an innovative accelerator that leverages a novel spatial array termed Nest and a novel multi-stage reduction network called BIRRD for performing flexible data reduction with layout reordering under the hood, enabling seamless switching between optimal dataflows with negligible latency and resources overhead. For systematically evaluating the performance interaction between dataflows and layouts, we enhance Timeloop, a state-of-the-art dataflow cost modeling and search framework, with layout assessment capabilities, and term it as Layoutloop. We model FEATHER into Layoutloop and also deploy FEATHER end-to-end on the edge ZCU104 FPGA. FEATHER delivers 1.27~2.89x inference latency speedup and 1.3~6.43x energy efficiency improvement compared to various SoTAs like NVDLA, SIGMA and Eyeriss under ResNet-50 and MobiletNet-V3 in Layoutloop. On practical FPGA devices, FEATHER achieves 2.65/3.91x higher throughput than Xilinx DPU/Gemmini. Remarkably, such performance and energy efficiency enhancements come at only 6% area over a fixed-dataflow Eyeriss-like accelerator. Our code is released at https://github.com/maeri-project/FEATHER.

==> fig/layout_analysis.tex <==
% \begin{figure*}[t]
%     \centering
%     % \vspace{-3mm}
%     \fcolorbox{blue}{white}{
%       \begin{subfigure}{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{fig/ResNet50_global_vs_layout.pdf}
%          \caption{\revise{ResNet50 only has typical Conv2D, leading to unified slowdown}.}
%          \label{fig:resnet50_lambda}
%      \end{subfigure}
%      \begin{subfigure}{\columnwidth}
%          \centering
%         %  \includesvg[width=0.8\linewidth]{fig/SL.svg}
%          \includegraphics[width=\columnwidth]{fig/MobV3_global_vs_layout.pdf}
%          \caption{\revise{MobV3 requires more scattered accesses from Depth-wise Conv2D}.}
%          \label{fig:mobv3_lambda}
%      \end{subfigure}}
%     \vspace{-3mm}
%     \caption{\revise{Latency evaluation (\Accel v.s. SIGMA)}} %\TK{minor comment -- you dont need the data points connected by a line. Just use the markers. Usually a line connecting the points is to indicate extrapolation (eg if x axis is inj rate, 0.01 and 0.02 are points plotted and line between them extrapolates. But in this case x axis is distint layers}\JT{Thanks! Resolved}} 
%     \label{fig:accel_to_sigma}
%     \vspace{-6mm}
% \end{figure*}


% \begin{figure*}[t]
%     \centering
%     \vspace{-4mm}
%      \subfloat[ResNet50 only has typical Conv2D, leading to unified slowdown. \label{fig:resnet50_lambda}]{{\includegraphics[width=0.495\textwidth]{fig/ResNet50_global_vs_layout.pdf}}}
%     \vspace{-2mm}
%     \subfloat[MobV3 requires more scattered accesses from Depth-wise Conv2D. \label{fig:mobv3_lambda}]{{\includegraphics[width=0.49\textwidth]{fig/MobV3_global_vs_layout.pdf}}} 
%     \vspace{-4mm}
%     \caption{Latency evaluation (\Accel v.s. SIGMA)} 
%     \label{fig:accel_to_sigma}
%     \vspace{-6mm}
% \end{figure*}

% \insertWideFigureRatio{ResNet50_global_vs_layout}{Evaluation of different layouts on searched optimal mapping under no layout constraints on ResNet-50.}{0.5}
% \insertWideFigureRatio{MobV3_global_vs_layout}{Evaluation of different layouts on searched optimal mapping under no layout constraints on MobileNet-V3.}{0.5}

==> fig/rir.tex <==
\begin{figure*}[t]
    \centering
     \begin{subfigure}{0.48\linewidth}
         \centering
        %  \includesvg[width=0.8\linewidth]{fig/optimize.svg}
         \includegraphics[width=\linewidth]{fig/AFFT_RIR_cycle0.pdf}
         \caption{Reorder results from bottom \Accel DPE row during reduction.}
         \label{fig:cycle0}
     \end{subfigure}
     \begin{subfigure}{0.48\linewidth}
         \centering
        %  \includesvg[width=0.8\linewidth]{fig/SL.svg}
         \includegraphics[width=\linewidth]{fig/AFFT_RIR_cycle3.pdf}
         \caption{Reorder results from top \Accel DPE row during reduction.}
         \label{fig:cycle3}
     \end{subfigure}
     \vspace{-2mm}
     \caption{Example of reordering data in reduction to switch data layout ($HW$\textcolor{red}{\underline{$C$}} $\rightarrow$ $HC$\textcolor{red}{\underline{$W$}}), which RIR resolves hazard in \figref{fig:on_chip_reorder}.}
     \label{fig:rir_0_latency}
\end{figure*}


==> src/01-Abstract.tex <==
\begin{abstract}
\label{sec:abstract}
The inference of ML models composed of diverse structures, types, and sizes boils down to the execution of different dataflows (i.e. different tiling, ordering, parallelism, and shapes). Using the optimal dataflow for every layer of workload can reduce latency by up to two orders of magnitude over a suboptimal dataflow. Unfortunately, reconfiguring hardware for different dataflows involves on-chip data layout reordering and datapath reconfigurations, leading to non-trivial overhead that hinders ML accelerators from exploiting different dataflows, resulting in suboptimal performance. 
To address this challenge, we propose \Accel, an innovative accelerator that leverages a novel spatial array termed \nest and a novel multi-stage reduction network called \noc for performing flexible data reduction with layout reordering under the hood, enabling seamless switching between optimal dataflows with negligible latency and resources overhead. 
For systematically evaluating the performance interaction between dataflows and layouts, we enhance Timeloop, a state-of-the-art dataflow cost modeling and search framework, with layout assessment capabilities, and term it as Layoutloop. We model \Accel into Layoutloop and also deploy \Accel end-to-end on the edge ZCU104 FPGA. \Accel delivers $1.27\sim2.89\times$ inference latency speedup and $1.3\sim6.43\times$ energy efficiency improvement compared to various SoTAs like NVDLA, SIGMA and Eyeriss under ResNet-50 and MobiletNet-V3 in Layoutloop. On practical FPGA devices, \Accel achieves $2.65$/$3.91\times$ higher throughput than Xilinx DPU/Gemmini. 
Remarkably, such performance and energy efficiency enhancements come at 
only $6$\% area over a fixed-dataflow Eyeriss-like accelerator.
\end{abstract}

==> src/cover.tex <==
% {{We thank reviewers for detailed feedbacks. Questions and revised contents are categorized by color: \RevCom{Common Concern}
% \RevA{Reviewer A}
% \RevB{Reviewer B}
% \RevC{Reviewer C}
% \RevD{Reviewer D}
% \RevE{Reviewer E}

\textbf{Summary of Key Changes:}
New \figref{fig:sota_reordering_concept_cmp}  and \tabref{tab:comparision_reordering} in \secref{sec:reorder_analysis} to categorize existing layout reordering techniques; added edge TPU to \figref{fig:Latency_Comparison_LAMBDA_DPU}, added MTIA-like and TPUv4-like reordering support to \figref{fig:Compare_to_SoTA}; Takeaways added for \figref{fig:Motivation},\ref{fig:lambda_walk_through_example},\ref{fig:lambda_mappings},\ref{fig:Full_RIR_Example}; revised contents to clarify/address all questions below.

%\noindent \RevCom{\textbf{R-A,R-C,R-D: Additional experiments to compare with SoTA including MTIA, TPUv4 and other embedded systems?}}



\noindent \RevA{\textbf{RA: Compare against reordering support in MTIA, TPUv4.}}
We have added \figref{fig:sota_reordering_concept_cmp} and \tabref{tab:comparision_reordering} to distinguish data reordering support provided by FEATHER vs. Medusa, TPUv4 and MTIA.  We also reached out to the TPU and MTIA teams at Google and Meta to confirm the functionality of their layout transformation support, and did a best effort implementation to contrast against them in new \figref{fig:Compare_to_SoTA}.
%
Specifically, (i) they perform ``on-chip reorder" as an additional step, while FEATHER does it during computation. (ii) they support a limited set of layout transformations, restricting dataflows they can efficiently support. %\PC{are you referring transformation as layout conversion?}
\textbf{\textit{We re-iterate that FEATHER is the first work to enable arbitrary data layout and dataflow transformations}}.


\noindent \RevA{\textbf{RA: are there potentially superior dataflows that haven't been covered previously for lack of layout evaluation?}} Yes, Layoutloop enables \textbf{dataflow/layout co-searching}, revealing that optimal dataflows identified without considering layout impacts perform poorly in practice, as illustrated in \figref{fig:per_layer_latency}. By incorporating layout effects, we discover superior dataflows that were previously non-optimal without factoring layout. %we find the resulted optimal dataflows performs severly bad in practice, if searching ignores layout effect, as shown in \figref{fig:per_layer_latency}. And thus other superior dataflows are found when factoring layout. % without layout evaluations are different and \figref{fig:per_layer_latency} demonstrates the performance gap of potentially superior dataflows with layout evaluation.

\noindent \RevB{\textbf{RB: Differences between on-the-fly input reordering (e.g. im2col) and the proposed Reordering in Reduction (RIR)?}}
%
We now clarify in \secref{sec:reorder_analysis}.
``Input Reordering" (e.g., Im2col, transpose in MTIA, row-reorder in TPU shown in \tabref{tab:comparision_reordering}) rearranges data before computation, leading to bank conflicts when layout is discordant and lacking flexibility for arbitrary layout transformation, shown in \figref{fig:line_rotation}, \ref{fig:transpose}, \ref{fig:row_reorder}. % read data from buffer, modify layouts and then feed reordered data into computation. This approach suffers from bank conflicts when layout is not concordant. And such approach cannot always guarantee concordant layout for lack of arbitrary reordering capability.
The proposed RIR or ``Output Reordering" reorders data during the reduction phase, aligning output directly to the next layer's layout requirements, thereby eliminating bank conflicts (\figref{fig:arbitrary_reorder})
% In proposed RIR or ``Output Reordering", reordering happens during the reduction phase of computation, 
% and writing output results to expected locations for desired concordant layout for next layer, and thus remove bank conflicts.
% modifies input data layouts before computation
%E.g., im2col converts CONV operations to matrix multiplication 
%(\tabref{tab:comparision_reordering}). %, while ``Output reordering"  adjusts the layouts of final results after computation. 
%This approach faces the challenge of bank conflicts due to concurrent on-chip buffer access.
%%%%% It does NOT decrease \textbf{concurrent on-chip buffer access}, thus not contributing to minimize bank conflicts.
% The proposed RIR or ``Output Reordering" reduces concurrent on-chip buffer access, key cause to bank conflicts, by accumulating many data into fewer results and then reordering these fewer results.

%. Because the reduction leads to fewer buffer accesses by accumulating partial sums into fewer results, and reordering achieves the desired layout by writing final results to expected location.
%In contrast, our proposed Reorder in Reduction (RIR) during computation, specifically in the reduction phase when partial sums are accumulated fewer final results such that reordering will have less number of buffer accesses and thus reduces bank conflicts. The desired layout is achieved when directly writing final results back.

% Im2col rearranges input data before processing to ease convolution operations using batch matrix multiplication. It reads input data from on-chip buffer, changing their layout and then feeding computation. Conversely, output reordering techniques alter layouts of output tensors after compute. Both do not change the number of data access to on-chip buffers, while our proposed Reduction in Reduction (RIR) reduces such data access by adjusting tensor layouts during the computation itself, specifically within the reduction phase, such that RIR reorders fewer data to on-chip buffer in desired layout.

% On-the-fly input reordering, like im2col, does \textbf{NOT} reduce the number of data or change the locations of data required from on-chip buffer. In contrast, RIR accumulates input partial sums into fewer final results and thus lessens output buffer port requirements, thereby significantly reducing bank conflicts. Additionally, while im2col mainly targets sliding-window parallelism, RIR supports parallelism in combination of sliding windows, channels, and kernels. 

 % \PC{Im2col is a method for rearranging input data to facilitate convolution operations by employing batch matrix multiplication. This technique involves transforming input tensors, with layout conversion occurring prior to computation. Conversely, output reordering techniques concentrate on altering the layouts of output tensors post-computation. In contrast, the proposed Reduction in Reduction (RIR) performs layout adjustments during the reduction process as part of the computation to achieve the desired output layout.} \JT{Thanks so much for the high-level suggestion! I incorporate and further I feel like this answer only introduces difference without saying benefits from such differences. Therefore, I further polish it up into the following }\JT{Thanks so much for the high-level suggestion! I incorporate and further I feel like this answer only introduces difference without saying benefits from such differences. Therefore, I further polish it up shown above}

\noindent \RevB{\textbf{RB: Experiment does not showcase “FEATHER with RIR generates a desirable layout for the next layer”}}
%
The bank conflict latency (red bar in \figref{fig:Compare_to_SoTA}) for FEATHER is zero across all workloads, demonstrating that FEATHER with RIR consistently generates desirable layouts for dataflows of all layers. We clarify this in \secref{sec:layout_loop_res}.

\noindent \RevB{\textbf{RB: How to search dataflow (and layout) for FEATHER?}}
%
We use {Timeloop's native mapper} for performing dataflow search.
We also {add layout modeling} support to Timeloop. 
%Timeloop performs ``internal hybrid search algorithm (exhaustive + search-space pruning)." to explore dataflows under ideal layout assumptions. We augments it into Layoutloop with practical layout assessments, and employ Layoutloop to search dataflows while considering layout impacts.
The search space, algorithm, and metrics are detailed in \secref{sec:vi_a}.
% \PC{rephrase this.}\JT{Done}


\noindent \RevB{\textbf{RB: How does global wiring in the PE column affect clock frequency compared to local connection in Systolic Array?}}
%In our experiments, 
We found the critical path to be inside the PE, not the global wires forwarding local results to the external reduction network. This is consistent with works like Eyeriss where data was broadcast in one cycle across the entire row of a 2D array. 
If the global wire does become a bottleneck (e.g., if the array is too large), we can pipeline it, maintaining FEATHER's functionality and throughput efficiency. We clarify this in \secref{sec:timing_analysis}.
% 
%In FEATHER, global wiring has negligible effects on maximal achievable clock frequency of systolic array, because timing critical path is wire connecting local weight registers to the multiplier of PE. Both FEATHER and GEMMINI achieve 1.5 GHz clocking under TSMC's 28nm, as detailed in \secref{sec:timing_analysis}.
%
%If the global wire does become a bottleneck (if the array is too large), we can pipeline it, maintaining FEATHER's functionality and throughput efficiency. 

% \PC{Sounds suspicious. In my experience, its the other way around. Neverthless, you can tone it down by saying less impact or neglibile impact.}\JT{Thanks! adopted the suggestion}

\noindent \RevB{\textbf{RB: The reason for higher frequency of FEATHER with global wiring than GEMMINI with local wiring in}} \tabref{tab:evaluation_setup}
%
Both FEATHER and GEMMINI achieve 1 GHz under TSMC's 28nm.
However, on FPGA devices, the FireSim toolchain  on AWS-F1 limits the maximal achievable clock frequency of GEMMINI at 50 MHz (\secref{sec:vi_a}). For fair comparison, we normalize throughput by number of PE and clock frequency.
% The frequencies in \tabref{tab:evaluation_setup} for FPGA devices are set solely for a fair comparison and do not represent the maximum achievable clock frequencies on ASICs. 
%We clarify it in .

\noindent \RevC{\textbf{RC: Did FEATHER use HLS optimization engine to perform static data layouts to provide an optimized baseline?}}
%
We use Xilinx Vitis HLS for optimized invocation of Xilinx IPs (clarified now in \secref{sec:vi_a}). We leverage Layoutloop to co-search dataflow/layout as discussed in RB. 

\noindent \RevC{\textbf{RC: Comparison against other embedded systems.}}
%
We now include end-to-end comparison of performance against Google's Coral Edge TPU in \secref{sec:edge_tpu_cmp} and updated \figref{fig:Latency_Comparison_LAMBDA_DPU}.

\noindent \RevC{\textbf{RC: How does the Multi-Dimensional-Access (MDA) memory affect FEATHER's benefits?}}
%
MDA supports both row-wise and column-wise access, akin to a layout transpose (\figref{fig:sota_reordering_concept_cmp}), mitigating but not entirely eliminating bank conflicts. FEATHER's benefits would remain valid even with MDA.
%to further minimize bank conflicts.
% MDA enables access in both row-wise and column-wise manners, similar to layout transpose, thereby reducing but not eliminating bank conflicts. FEATHER's benefits remain valid to further augment MDA to avoid bank conflicts.

% FEATHER enables future software optimizations by supporting run-time dynamic dataflow and layout switching. 
% Taking dynamic shapes arising from mixture of experts in Transformer models as an example. One of SW optimizations could be dynamically selecting best dataflow for an operation with dynamic shapes at runtime. FEATHER enables such an optimization by enhancing runtime for dynamic selection without any hardware changes.
% This adaptability facilitates the development of new dataflows and layouts, ensuring FEATHER remains compatible with future software advancements.
% While current compilers focus on general optimizations across various devices, FEATHER paves the way for more specialized optimizations tailored to flexible hardware and dynamic workload shapes. 

% FEATHER enables exploration in dataflow and layout design spaces through its fully flexible architecture, supporting current and potential future software enhancements.
% \PC{I think we need a better answer here.}\JT{I redraft a new answer, any feedback will be appreciated}

\noindent \RevC{\textbf{RC: Compare against reordering support in MTIA, TPUv4.}}
See RA above.

\noindent \RevC{\textbf{RC: how FEATHER provision for future SW optimizations?}}
%
FEATHER ensures adaptability for future SW optimizations by allowing dynamic dataflow \& layout \textbf{adjustments at runtime without hardware changes} w/ examples below.%or example, as for dynamic shapes arising from mixture of experts in Transformer models,  potential SW optimizations could be dynamically selecting best dataflow for an operation with dynamic shapes at runtime. Such optimizations boil down to enhance runtime for dynamic selection with no changes to hardware.

\noindent \RevD{\textbf{RD: FEATHER indicates meagre speedups than Medusa variant of SIGMA in results section}} (\secref{sec:timing_analysis})
%
Modest speedups only occur when operator shape aligns with parallelism of HW under concordant layout (e.g., ResNet-50). But on workloads with skewed operators (e.g., MobileNet-V3), FEATHER achieves $1.18\times$ speedup with $1.85\times$ efficiency (\secref{rev:prior_fgpa_accel}).

% \footnote{\RevD{Such modest speedup only happens when workload sizes precisely align with the layout and hardware parallelism. However, modern workloads often do not match hardware parallelism. In such irreuglar scenario, as shown by MobileNet-V3 in }\figref{fig:Compare_to_SoTA}\RevD{, FEATHER reduces latency by 18\% and energy consumption by 85\%, and saves 73.6\% area compared to the Medusa variant of SIGMA, underscoring FEATHER's superiority and necessity.}}

% observed with ResNet-50 occur because the workload size precisely aligns with the layout and hardware parallelism, making even static layouts without reordering nearly as effective as designs with line rotation. However, modern workloads often do not match hardware parallelism. In such irreuglar scenario, as shown by MobileNet-V3 in \figref{fig:Compare_to_SoTA}, FEATHER reduces latency by 18\% and energy consumption by 85\%, and saves 73.6\% area compared to the Medusa variant of SIGMA, underscoring FEATHER's superiority and necessity in handling such scenarios. We revised in \secref{rev:prior_fgpa_accel}.


\noindent \RevD{\textbf{RD: Limitation of offline optimization for dataflow-layout pairs.}}
%each layer's layout to select the optimal dataflow-layout pair for new workloads.}}
%Is this a limitation?}}
%
%FEATHER's dataflow/layout searching happens offline. %, as good as SotA Timeloop searching (multithreading random search constrained on search size and victory conditions). 
These are one-time costs for all future inferences.

\noindent \RevE{\textbf{RE: Support for dynamic structures and shapes like MoE?}}
%
MoE's dynamic nature can be addressed by compiling for all potential layer orders and shapes, with runtime selection of optimal configurations. To reduce compilation time, we may consider only the maximal shape values, ensuring FEATHER remains efficient and adaptable to dynamic scenarios.
%


\noindent \RevE{\textbf{RE: Compiler and runtime modifications for arbitrary dataflows?}}
%
To support arbitrary dataflow parallelism without explicit layout conversion operations, we modified our compiler by eliminating layout exploration from the graph optimizer and introducing Layoutloop in the kernel optimizer for integrated dataflow + layout optimization.
%
Layoutloop currently supports only static shapes (dynamic shapes planned for future work). 
No runtime modifications were necessary as these optimizations occur at compile-time for known static shapes.


\noindent \RevE{\textbf{RE: How is ping-pong buffer managed?}}
%By compiler, runtime, or both?}}
Ping-pong buffer switching scheduling is managed by the compiler with the goal to improve array utilization, similar to scratchpad management in DNN accelerators today.%\JT{I get confused on whether our response answers the question of reviewer, any comments are appreciated.} 
% \PC{In the slack, the posted question was "how does the current compiler handles flexible dataflows/layout"? We need to modify the text for the above inter-layer pipelining and ping-ping stuff.}\JT{I corrected ping-pong with previous answers.}


\noindent \RevE{\textbf{RE: Does the RIR reordering impact numerical accuracy or stability of computations?}}
%
No. RIR simply does reordering of the data to be written to the scratchpad, and does not change final value of accumulated partial sums.

\noindent \RevE{\textbf{RE: End-to-end performance impact of bank conflicts?}}
%
%Bank conflicts introduce pipeline stall in computation engine, leading to under utilization.
We now quantify 
%end-to-end performance impact of bank conflicts slowdown 
this as red bar in \figref{fig:Compare_to_SoTA}.

% to improve accessibility for a wider audience and paper flow.



% \textbf{!!The below are original questions and answers. I merged following two questions and answers together!!}

% \noindent \RevE{\textbf{RE: Does the assumption of deterministic inter-layer dataflow patterns in FEATHER limit its effectiveness for dynamic structures and shapes like those in large language models (LLMs), specifically mixture-of-experts (MoE)?}}

% MoE's dynamic nature is addressed by compiling for all potential layer orders and shapes, with runtime selection of optimal configurations. To reduce compilation time, we may consider only the maximal shape values, ensuring FEATHER remains efficient and adaptable to dynamic scenarios.
% % Current dataflow-layout co-searching via Layoutloop assumes static tensor shapes, which could be augmented to MoE by taking maximal sizes of dynamic shapes into exploration. %However, this doesn't restrict the FEATHER capabilities of supporting MoE because dataflow exploration is done at compile time.  
% % \PC{Please include my comments from HackMd. The reviewer is referring to dynamic tensor shapes and LayoutLoop cannot handle that.}\JT{Done}

% \noindent \RevE{\textbf{RE: The evaluation could benefit from more specifics regarding compiler and runtime modifications needed to support arbitrary dataflow parallelism and dynamic shapes.}}

% To support arbitrary dataflow parallelism without explicit layout conversion operations, we modified our compiler by eliminating layout exploration from the graph optimizer and introducing LayoutLoop in the kernel optimizer for integrated dataflow + layout optimization. LayoutLoop currently supports only static shapes, with dynamic shapes planned for future work. No runtime modifications were necessary as these optimizations occur at compile-time for known static shapes.

